$\mu$Tiles: Efficient Intra-Process Privilege Enforcement of Memory Regions

With the alarming rate of security advisories and privacy concerns on connected devices, there is an urgent need for strong isolation guarantees in resource-constrained devices that demand very lightweight solutions. However, the status quo is that Unix-like operating systems do not offer privilege separation inside a process. Lack of practical fine-grained compartmentalization inside a shared address space leads to private data leakage through applications' untrusted dependencies and compromised threads. To this end, we propose $\mu$Tiles, a lightweight kernel abstraction and set of security primitives based on mutual distrust for intra-process privilege separation, memory protection, and secure multithreading. $\mu$Tiles takes advantage of hardware support for virtual memory tagging (e.g., ARM memory domains) to achieve significant performance gain while eliminating various hardware limitations. Our results (based on OpenSSL, the Apache HTTP server, and LevelDB) show that $\mu$Tiles is extremely lightweight (adds $\approx 10KB$ to kernel image) for IoT use cases. It adds negligible runtime overhead ($\approx 0.5\%-3.5\%$) and is easy to integrate with existing applications for providing strong privilege separation.

==> vs.tex <==

\begin{table*}[htb]
  \centering
  \footnotesize
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{|l|l|l|}
    \hline
    Feature                   & ARM Memory Domains                             & Intel MPK                                                            \\ \hline
    Per process domains       & 16                                             & 16                                                                   \\ \hline
    Access control register   & DACR  (2 bits per domain, privileged register) & PKRU (2 bits per domain, userspace register)                         \\ \hline
    Access rights             & No-access, Full access, MMU default            & No-access, write-disable, MMU default                                \\ \hline
    Paging modes              & 2-level paging (bits 8:5, level 1 entries)     &  4-level paging (bits 62:59 of PDPTE)                                \\ \hline
    Address space privilege   &  Privileged \& usersapce                       &  Userspace only                                                      \\ \hline
    Specific page fault       & Domain fault                                   & PK fault                                                             \\ \hline
    Kernel virtual memory API & No support                                     & Limited support (\texttt{pkey\_mprotect}, \texttt{pkey\_alloc}, \texttt{pkey\_free}, and \texttt{mmap}) \\ \hline
    \end{tabular}}

    \caption{ARM memory domains vs Intel MPK: Despite being efficient building blocks of isolation, such features have various limitations that \textmu Tiles abstraction resolves to provide effective intra-process privilege separation.}
    \label{mpk}
\end{table*}
